Process-Supervised LLM Recommenders via Flow-guided Tuning

While large language models (LLMs) are increasingly adapted for recommendation systems via supervised fine-tuning (SFT), this approach amplifies popularity bias due to its likelihood maximization objective, compromising recommendation diversity and fairness. To address this, we present Flow-guided fine-tuning recommender (Flower), which replaces SFT with a Generative Flow Network (GFlowNet) framework that enacts process supervision through token-level reward propagation. Flower's key innovation lies in decomposing item-level rewards into constituent token rewards, enabling direct alignment between token generation probabilities and their reward signals. This mechanism achieves three critical advancements: (1) popularity bias mitigation and fairness enhancement through empirical distribution matching, (2) preservation of diversity through GFlowNet's proportional sampling, and (3) flexible integration of personalized preferences via adaptable token rewards. Experiments demonstrate Flower's superior distribution-fitting capability and its significant advantages over traditional SFT in terms of accuracy, fairness, and diversity, highlighting its potential to improve LLM-based recommendation systems. The implementation is available via https://github.com/MrPeach0301/Flower

==> sections/author.tex <==

\author{Chongming Gao}
\email{chongming.gao@gmail.com}
\orcid{0000-0002-5187-9196}
\affiliation{%
  \institution{University of Science and Technology of China}
%   \streetaddress{P.O. Box 1212}
  \city{Hefei}
  \state{Anhui}
  \country{China}
%   \postcode{43017-6221}
}


\author{Kexin Huang}
\email{huangkx@mail.ustc.edu.cn}
\orcid{0009-0001-4868-0952}
\affiliation{%
  \institution{University of Science and Technology of China}
%   \streetaddress{P.O. Box 1212}
  \city{Hefei}
  \state{Anhui}
  \country{China}
%   \postcode{43017-6221}
}


\author{Zian Fei}
\email{feiziang@mail.ustc.edu.cn}
% \orcid{0000-0002-7849-208X}
\affiliation{%
  \institution{University of Science and Technology of China}
  \city{Hefei}
  \state{Anhui}
  \country{China}
}


\author{Jiaju Chen}
\email{cjj01@mail.ustc.edu.cn}
% \orcid{0000-0001-5667-5347}
\affiliation{%
  \institution{University of Science and Technology of China}
  \city{Hefei}
  \state{Anhui}
  \country{China}
}


\author{Jiawei Chen}
\email{sleepyhunt@zju.edu.cn}
\orcid{0000-0002-4752-2629}
\affiliation{%
  \institution{Zhejiang University}
%   \streetaddress{P.O. Box 1212}
  \city{Hangzhou}
  \state{Zhejiang}
  \country{China}
%   \postcode{43017-6221}
}


% \author{Peng Jiang}
% \email{jiangpeng@kuaishou.com}
% \orcid{0000-0002-9266-0780}
% \affiliation{%
%   \institution{Kuaishou Technology Co., Ltd.}
%   \country{}
% }

% \author{Shiqi Wang}
% \email{shiqi@cqu.edu.cn}
% \orcid{0000-0002-5369-884X}
% \affiliation{%
%   \institution{Chongqing University}
%   \city{Chongqing}
%   \country{China}
% }

% \author{Zhong Zhang}
% \email{zhongzhang@std.uestc.edu.cn}
% \orcid{0000-0003-1349-9755}
% \affiliation{%
%   \institution{University of Electronic Science and Technology of China}
%   \country{}
% }


% \author{Xiangnan He}
% \authornotemark[1]
% \email{xiangnanhe@gmail.com}
% \orcid{0000-0001-8472-7992}
% \affiliation{%
%   \institution{University of Science and Technology of China}
%   \country{}
% }

\renewcommand{\shortauthors}{Chongming Gao et al.}

% \renewcommand{\shortauthors}{Gao et al.}

==> sections/definition.tex <==
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    Bib\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
\setcopyright{acmcopyright}
\copyrightyear{2018}
\acmYear{2018}
\acmDOI{XXXXXXX.XXXXXXX}

%% These commands are for a PROCEEDINGS abstract or paper.
\acmConference[Conference acronym 'XX]{Make sure to enter the correct
  conference title from your rights confirmation emai}{June 03--05,
  2018}{Woodstock, NY}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}



\usepackage{booktabs}
\usepackage{multirow}
\usepackage{url}
\usepackage{enumitem}   
\usepackage{float} % For figure floating in appendix
\usepackage{colortbl} % 引入colortbl包
\definecolor{mygray}{rgb}{0.9, 0.9, 0.9}




\definecolor{myred}{rgb}{0.68627451, 0.14117647, 0.09803922}

% Added automatically
% \newcommand{\myeq}[1]{\hyperref[eq:#1]{Equation~(\ref*{eq:#1})}}
\newcommand{\myeq}[1]{\hyperref[eq:#1]{Eq.~(\ref*{eq:#1})}}
\newcommand{\mysec}[1]{\hyperref[sec:#1]{Section~\ref*{sec:#1}}}
\newcommand{\mytable}[1]{\hyperref[tab:#1]{Table~\ref*{tab:#1}}}
\newcommand{\myfig}[1]{\hyperref[fig:#1]{Fig.~\ref*{fig:#1}}}
\newcommand{\myappendix}[1]{\hyperref[appendix:#1]{Appendix~\ref*{appendix:#1}}}
% \newcommand{\myappendix}[1]{\hyperref[appendix:#1]{Appendix}}
\newcommand{\myalg}[1]{\hyperref[alg:#1]{Algorithm~\ref*{alg:#1}}}
\newcommand{\myhyp}[1]{\hyperref[hyp:#1]{\textsc{Hypothesis}~\ref*{hyp:#1}}}


\newcommand{\mytheorem}[1]{\hyperref[theorem:#1]{Theorem~\ref*{theorem:#1}}}
\newcommand{\mylemma}[1]{\hyperref[lemma:#1]{Lemma~\ref*{lemma:#1}}}
%



==> sections/meta.tex <==
% \copyrightyear{2022}
% \acmYear{2022}
% \setcopyright{acmcopyright}
% \acmConference[SIGIR '23] {Proceedings of the 46th International ACM SIGIR Conference on Research and Development in Information Retrieval}{July 23--27, 2023}{Taipei.}
% \acmBooktitle{Proceedings of the 46th International ACM SIGIR Conference on Research and Development in Information Retrieval (SIGIR '23), July 23--27, 2023, Taipei.}
% \acmPrice{15.00}
% \acmISBN{978-1-4503-9236-5/22/10}
% \acmDOI{10.1145/3511808.3557624}

% % SIGIR 23
% \copyrightyear{2023} 
% \acmYear{2023} 
% \setcopyright{acmlicensed}\acmConference[SIGIR '23]{Proceedings of the 46th
% International ACM SIGIR Conference on Research and Development in
% Information Retrieval}{July 23--27, 2023}{Taipei, Taiwan}
% \acmBooktitle{Proceedings of the 46th International ACM SIGIR Conference on
% Research and Development in Information Retrieval (SIGIR '23), July 23--27,
% 2023, Taipei, Taiwan}
% \acmPrice{15.00}
% \acmDOI{10.1145/3539618.3591636}
% \acmISBN{978-1-4503-9408-6/23/07}




\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002951.10003317.10003347.10003350</concept_id>
<concept_desc>Information systems~Recommender systems</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}
\ccsdesc[500]{Information systems~Recommender systems}


% %%
% %% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% %% Please copy and paste the code instead of the example below.
% %%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>00000000.0000000.0000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Do, Not, Us, This, Code, Put, the, Correct, Terms, for,
  Your, Paper}

% %% A "teaser" image appears between the author and affiliation
% %% information and the body of the document, and typically spans the
% %% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}

